Jitter Characterization of the HyTI Satellite

The Hyperspectral Thermal Imager (HyTI) is a technology demonstration mission that will obtain high spatial, spectral, and temporal resolution long-wave infrared images of Earth's surface from a 6U cubesat. HyTI science requires that the pointing accuracy of the optical axis shall not exceed 2.89 arcsec over the 0.5 ms integration time due to microvibration effects (known as jitter). Two sources of vibration are a cryocooler that is added to maintain the detector at 68 K and three orthogonally placed reaction wheels that are a part of the attitude control system. Both of these parts will introduce vibrations that are propagated through to the satellite structure while imaging. Typical methods of characterizing and measuring jitter involve complex finite element methods and specialized equipment and setups. In this paper, we describe a novel method of characterizing jitter for small satellite systems that is low-cost and minimally modifies the subject's mass distribution. The metrology instrument is comprised of a laser source, a small mirror mounted via a 3D printed clamp to a jig, and a lateral effect position-sensing detector. The position-sensing detector samples 1000 Hz and can measure displacements as little as 0.15 arcsec at distances of one meter. This paper provides an experimental procedure that incrementally analyzes vibratory sources to establish causal relationships between sources and the vibratory modes they create. We demonstrate the capabilities of this metrology system and testing procedure on HyTI in the Hawaii Space Flight Lab's clean room. Results include power spectral density plots that show fundamental and higher-order vibratory modal frequencies. Results from metrology show that jitter from reaction wheels meets HyTI system requirements within 3$\sigma$.

==> tab-freqs-found.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[hbt!]
\label{tab:freqs_found}
\caption{List of modes associated with the vibratory source.}
\renewcommand*{\arraystretch}{1.3}
\begin{center}
\begin{tabular}{|c|c|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Vibratory Source}} & \multicolumn{1}{c|}{Identified Modes in-track (Hz)} \\ \cline{2-2} 
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{Identified Modes Across-Track (Hz)} \\ \hline
\multirow{2}{*}{Cryocooler and Camera (Payload)} & \begin{tabular}[c]{@{}l@{}}16, 60, 120, 180, 240, 300, 340, 360\\ 420, 460, 480\end{tabular} \\ \cline{2-2} 
 & \begin{tabular}[c]{@{}l@{}}35, 70, 97, 106, 120, 140, 180,\\ 212, 240, 276, 325\end{tabular} \\ \hline
\multirow{2}{*}{Reaction Wheels: x-direction at 3000 rpm} & None detected \\ \cline{2-2} 
 & None detected \\ \hline
\multirow{2}{*}{Reaction Wheels: z-direction at 3000 rpm} & None detected \\ \cline{2-2} 
 & 11, 58 \\ \hline
\multirow{2}{*}{Reaction Wheels: x- and z-direction at 3000 rpm} & 208, 368 \\ \cline{2-2} 
 & 10, 58, 208 \\ \hline
\end{tabular}
\end{center}
\end{table*}

==> tab-modes_found.tex <==
\begin{table}[hbt!]
\centering
\begin{tabular}{c|c|c|}
\cline{2-3}
Configuration &
  \begin{tabular}[c]{@{}c@{}}In-Track Modes \\ Identified (Hz)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Across-Track Modes \\ Identified (Hz)\end{tabular} \\ \hline
\multicolumn{1}{|c|}{\textcircled{1}} &
  240, 324 &
  \begin{tabular}[c]{@{}c@{}}35, 70, 97, 106, 120, 139 , \\ 179, 211, 240, 275, 324\end{tabular} \\ \hline
\multicolumn{1}{|c|}{\textcircled{2}} &
  \begin{tabular}[c]{@{}c@{}}16, 60, 120, 180, 240, 300, \\ 340, 360, 420, 460, 480\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}34, 60, 93, 120, 180, 240,\\ 300, 360, 460, 480\end{tabular} \\ \hline
\multicolumn{1}{|c|}{\textcircled{3}} & 120            & 120         \\ \hline
\multicolumn{1}{|c|}{\textcircled{4}} & 120            & 120         \\ \hline
\multicolumn{1}{|c|}{\textcircled{5}} & 0.03           & 11, 58      \\ \hline
\multicolumn{1}{|c|}{\textcircled{6}} & 0.02, 208, 368 & 10, 58, 208 \\ \hline
\end{tabular}
\end{table}
